nicolay-r at SemEval-2024 Task 3: Using Flan-T5 for Reasoning Emotion Cause in Conversations with Chain-of-Thought on Emotion States

Emotion expression is one of the essential traits of conversations. It may be self-related or caused by another speaker. The variety of reasons may serve as a source of the further emotion causes: conversation history, speaker's emotional state, etc. Inspired by the most recent advances in Chain-of-Thought, in this work, we exploit the existing three-hop reasoning approach (THOR) to perform large language model instruction-tuning for answering: emotion states (THOR-state), and emotion caused by one speaker to the other (THOR-cause). We equip THOR-cause with the reasoning revision (rr) for devising a reasoning path in fine-tuning. In particular, we rely on the annotated speaker emotion states to revise reasoning path. Our final submission, based on Flan-T5-base (250M) and the rule-based span correction technique, preliminary tuned with THOR-state and fine-tuned with THOR-cause-rr on competition training data, results in 3rd and 4th places (F1-proportional) and 5th place (F1-strict) among 15 participating teams. Our THOR implementation fork is publicly available: https://github.com/nicolay-r/THOR-ECAC

==> tables/emotion_state_method_analysis.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|cc}
    \hline
    Method & Accuracy & F1 \\
    \hline
    Zero-shot & & \\
    \hline
    ChatGPT-3.5-0613                    &  0.533	 &         \\
    Mistral-instruct-v0.2               &  0.506	 &         \\ 
    \hline
    Fine-tuning & & \\
    \hline
    Flan-T5\textsubscript{base} (THoR)  &  \textbf{0.62} & \textbf{47.81}  \\
    % Flan-T5\textsubscript{large} (THoR) &  0.64	     & 51.195  \\
    \hline
    \end{tabular}
    \caption{Results for Emotion States Prediction analysis on ... dataset. \textcolor{red}{This table is like gonna be excluded from the paper.}}
    \label{tab:emotion-state-analysis}
\end{table}
